Identification of Background False Positives from Kepler Data

The Kepler Mission was launched on March 6, 2009 to perform a photometric survey of more than 100,000 dwarf stars to search for Earth-size planets with the transit technique. The reliability of the resulting planetary candidate list relies on the ability to identify and remove false positives. Major sources of astrophysical false positives are planetary transits and stellar eclipses on background stars. We describe several new techniques for the identification of background transit sources that are separated from their target stars, indicating an astrophysical false positive. These techniques use only Kepler photometric data. We describe the concepts and construction of these techniques in detail as well as their performance and relative merits.

==> fp_figures.tex <==
\input{APOvsGalLat.tex}
\input{collectedPixelFigure.tex}
\input{rainPlotFigures.tex}
\input{foldedCentroiMotionFigures.tex}
\input{koi1860FwAnalysisFigures.tex}
\input{fwCentroidsSourceLocation.tex}
\input{centroidedPixelsFigure.tex}
\input{fluxOvershootFigure.tex}
\input{koi_221_109_diff_images.tex}
\clearpage
\input{koi_2949_diff_image.tex}
\input{koi_221_cadences.tex}
\input{kepler_11_transit_interference.tex}
\input{koi_1861_diff_image.tex}
\input{koi_1860_diff_image.tex}
\input{combining_quarters_figures.tex}
\input{quarter_average_figures.tex}
\clearpage
\input{pixel_correlation_figures.tex}
\input{koi_975_diff.tex}
\input{accuracy_figures_1.tex}
\input{accuracy_figures_2.tex}
\clearpage
\input{accuracy_figures_3.tex}
\input{offset_vs_snr_figure.tex}
\input{PRF_vs_fw_offset_figure.tex}
\clearpage
\input{prf_offset_vs_offset_in_sigma_figure.tex}
\input{fw_offset_vs_offset_in_sigma.tex}
\input{prf_offset_vs_offset_in_sigma_augment.tex}

